Increasing tableaux and Narayana numbers

We give a counting formula for the set of rectangular increasing tableaux in terms of generalized Narayana numbers. We define small $m$-Schr\"oder paths and give a bijection between the set of increasing rectangular tableaux and small $m$-Schr\"oder paths, generalizing a result of Pechenik [3]. Using $K$-jeu de taquin promotion, which was defined by Thomas and Yong [10], we give a cyclic sieving phenomenon for the set of increasing hook tableaux.

==> smallschroder-30.tex <==
\psset{unit=8mm}
\begin{center}\begin{pspicture}(-1,-1)(5,5)
 \psset{linewidth=.5pt}
  \psline{->}(0,0)(4.5,0)\psline{->}(0,0)(0,4.5)
  \psline[linestyle=dotted](0,0)(4,4)
 \psset{linewidth=.2pt}
  \multips(0,0)(0,1){5}{\psline(4,0)}
  \multips(0,0)(1,0){5}{\psline(0,4)}
 \psset{linewidth=1.6pt}  
  \psline(0,0)(1,0)(1,1)(2,1)(4,3)(4,4) 
  \pscircle*(0,0){.1}\pscircle*(4,4){.1}
  \rput[tr](-.1,-.1){\small $(0,0)$}\rput[bl](4.1,4.1){\small $(4,4)$}
\end{pspicture}\end{center}

